Measurements of the E-Mode Polarization and Temperature-E-Mode Correlation of the CMB from SPT-3G 2018 Data

We present measurements of the $E$-mode ($EE$) polarization power spectrum and temperature-$E$-mode ($TE$) cross-power spectrum of the cosmic microwave background using data collected by SPT-3G, the latest instrument installed on the South Pole Telescope. This analysis uses observations of a 1500 deg$^2$ region at 95, 150, and 220 GHz taken over a four month period in 2018. We report binned values of the $EE$ and $TE$ power spectra over the angular multipole range $300 \le \ell < 3000$, using the multifrequency data to construct six semi-independent estimates of each power spectrum and their minimum-variance combination. These measurements improve upon the previous results of SPTpol across the multipole ranges $300 \le \ell \le 1400$ for $EE$ and $300 \le \ell \le 1700$ for $TE$, resulting in constraints on cosmological parameters comparable to those from other current leading ground-based experiments. We find that the SPT-3G dataset is well-fit by a $\Lambda$CDM cosmological model with parameter constraints consistent with those from Planck and SPTpol data. From SPT-3G data alone, we find $H_0 = 68.8 \pm 1.5 \mathrm{km\,s^{-1}\,Mpc^{-1}}$ and $\sigma_8 = 0.789 \pm 0.016$, with a gravitational lensing amplitude consistent with the $\Lambda$CDM prediction ($A_L = 0.98 \pm 0.12$). We combine the SPT-3G and the Planck datasets and obtain joint constraints on the $\Lambda$CDM model. The volume of the 68% confidence region in six-dimensional $\Lambda$CDM parameter space is reduced by a factor of 1.5 compared to Planck-only constraints, with only slight shifts in central values. We note that the results presented here are obtained from data collected during just half of a typical observing season with only part of the focal plane operable, and that the active detector count has since nearly doubled for observations made with SPT-3G after 2018.

==> nuisance_param_table.tex <==
\begin{table}[ht!]
\def\arraystretch{1.5}
\small
\setlength{\tabcolsep}{10pt}
\centering
\begin{tabular}{l c  c}
\hline\hline
 Parameter & Prior & Fit Value\\
 \hline
 $100\kappa$ & $0 \pm 0.045$ & $0.002 \pm 0.046$\\
 $A^{\EE}_{80}$ &$0.0133 \pm 0.0040$ & $0.014 \pm 0.004$\\
 $\alpha^{\EE}_{80}$ & $-2.42 \pm 0.02$ & $-2.419 \pm 0.020$\\
% $\alpha^{\TE}_{80}$ & $-2.42 \pm 0.02$ & $-2.420 \pm 0.021$\\
 $D^\mathrm{ps,~95\times95}_{3000}$ &  $0.0405 \pm 0.0121$ & $0.041 \pm 0.012$\\
 $D^\mathrm{ps,~150\times150}_{3000}$ & $0.0115 \pm 0.0034$ & $0.012 \pm 0.005$\\
 $D^\mathrm{ps,~220\times220}_{3000}$ & $0.0476 \pm 0.0143$ & $0.048 \pm 0.015$\\
 $D^\mathrm{ps,~95\times150}_{3000}$ & $0.0180 \pm 0.0054$ & $0.018 \pm 0.006$\\
 $D^\mathrm{ps,~95\times220}_{3000}$ & $0.0157 \pm 0.0047$ & $0.016 \pm 0.006$\\
 $D^\mathrm{ps,~150\times220}_{3000}$ & $0.0190 \pm 0.0057$ & $0.019 \pm 0.006$\\
 $T\strut^{\,95}_\mathrm{cal}$ & 0.85 -- 1.15 & $1.000 \pm 0.012$\\
 $T\strut^{\,150}_\mathrm{cal}$ & 0.85 -- 1.15 & $0.993 \pm 0.010$\\
 $T\strut^{\,220}_\mathrm{cal}$ & 0.85 -- 1.15 & $1.007 \pm 0.025$\\
 $P\strut^{\,95}_\mathrm{cal}$ & $0.9941 \pm 0.0088$ & $1.000 \pm 0.008$\\
 $P\strut^{\,150}_\mathrm{cal}$ & $0.9955 \pm 0.0082$ & $0.998 \pm 0.008$\\
 $P\strut^{\,220}_\mathrm{cal}$ & $0.9880 \pm 0.0182$ & $1.004 \pm 0.010$\\
\hline
\end{tabular}
\caption[
Priors and fit values of foreground and instrumental nuisance parameters
]{
Priors and fit values for the foreground and instrumental nuisance parameters describing mean-field lensing convergence $\kappa$, the amplitude $A^{XY}_{80}$ (in $\mu$K$^2$) and spectral index $\alpha^{XY}_{80}$ of polarized galactic dust, the $\EE$ power of Poisson-distributed point sources $D_{3000}^{\mathrm{ps,~\nu_i\times\nu_j}}$ (in  $\mu$K$^2$), absolute temperature calibration factor $T_\mathrm{cal}^{\nu_i}$, and absolute polarization calibration factor $P_\mathrm{cal}^{\nu_i}$.
}
\label{tab:nuisance_param_table}
\end{table}

